Massively multiplayer browser games on stateless pages and a relational database, a tutorial on their construction

A massively multiplayer browser game is a persistent world that many players change through ordinary web pages, with no client to install. This work is a tutorial for a developer or developer who wants to structure such a game from the start, from the overall organisation into modules to the protocols between players. The running example is the open-source role-playing game Naruto! Nigeru, whose engine keeps the whole game state in a relational database and uses no third-party library. The tutorial presents the overall view of the game, how its code is separated into modules, which technologies it uses and which ones it avoids, and then each mechanism as a design decision with its alternatives, namely the request cycle, the data model, the identity of the player without sessions, the world map computed from a hash of the coordinates, the turn-based combat, the economy under simultaneous requests, the trade and duel protocols, the ways a page waits for another player, and the content and languages. It closes with a suggested order of construction and the lessons of the example. The example has 25,930 lines of code in 9 feature modules over a core of 2,364 lines.

==> tables/c2.tex <==
\begin{table*}[t]
\centering
\caption{Repetitions out of 30 in which the conserved quantity changed when $N$ identical transfer requests were released at the same instant.}
\label{tab:c2}
\begin{tabular}{llrrrrrrr}
\toprule
System & Operation & $N=2$ & $N=4$ & $N=8$ & $N=16$ & $N=32$ & Max $|\Delta|$ & Burst (ms) \\
\midrule
\textbf{Nigeru~RPG}$^{*}$ & donate money & 0 & 0 & 0 & 0 & 0 & 0 & 694 \\
 & donate from bank & 0 & 0 & 0 & 0 & 0 & 0 & 2,206 \\
 & send banked item & 0 & 0 & 0 & 0 & 0 & 0 & 2,102 \\
 & bank deposit & 0 & 0 & 0 & 0 & 0 & 0 & 176 \\
 & bank withdrawal & 0 & 0 & 0 & 0 & 0 & 0 & 2,226 \\
\midrule
Shinobi Chronicles~\cite{elementum2026shinobi} & send money & 0 & 0 & 0 & 0 & 0 & 0 & 868 \\
\midrule
Legend of the Green Dragon~\cite{nbcore2026lotgd} & bank transfer & \textbf{30} & \textbf{30} & \textbf{30} & \textbf{30} & \textbf{30} & 8,100 & 5,865 \\
 & bank transfer, guarded & 0 & 0 & 0 & 0 & 0 & 0 & 5,126 \\
 & bank deposit & 0 & 0 & 0 & 0 & 0 & 0 & 5,759 \\
 & bank deposit, guarded & 0 & 0 & 0 & 0 & 0 & 0 & 5,175 \\
 & bank withdrawal & 0 & 0 & 0 & 0 & 0 & 0 & 5,778 \\
 & bank withdrawal, guarded & 0 & 0 & 0 & 0 & 0 & 0 & 5,107 \\
\midrule
TravianZ~\cite{shadowss2026travianz} & send resources & 0 & \textbf{30} & \textbf{30} & \textbf{30} & \textbf{30} & 9,500 & 641 \\
\bottomrule
\end{tabular}
\begin{tablenotes}
\item $^{*}$ System presented in this work. Max $|\Delta|$ is the largest absolute change of the conserved quantity, namely the money, items or resources summed over the accounts involved, in any repetition. Burst is the median time, at $N=32$, from the release of the requests to the end of the last response. Guarded denotes the optional transaction-based mode of Legend of the Green Dragon. Bold marks a nonzero count.
\end{tablenotes}
\end{table*}


==> tables/c4.tex <==
\begin{table}[t]
\centering
\caption{Character level of the 664 accounts of the original server.}
\label{tab:c4}
\begin{tabular}{lr}
\toprule
Statistic & Value \\
\midrule
Minimum & 1 \\
First quartile & 1 \\
Median & 1 \\
Third quartile & 1 \\
Maximum & 89 \\
Mean & 2.60 \\
Standard deviation & 6.37 \\
Accounts at level 5 or above & 69 \\
Accounts at level 10 or above & 35 \\
Accounts at level 20 or above & 16 \\
Accounts at level 30 or above & 7 \\
Accounts at level 50 or above & 2 \\
\bottomrule
\end{tabular}
\begin{tablenotes}
\item Quartiles by linear interpolation between the closest ranks. The standard deviation is the population standard deviation.
\end{tablenotes}
\end{table}


==> tables/features.tex <==
\begin{table}[t]
\centering
\caption{Selected game and engine features of the systems in comparison.}
\label{tab:features}
\setlength{\tabcolsep}{2.5pt}
\begin{tabular}{lcccccccc}
\toprule
Feature & \rotatebox{90}{\textbf{Nigeru}$^{*}$} & \rotatebox{90}{Shinobi~\cite{elementum2026shinobi}} & \rotatebox{90}{LotGD~\cite{nbcore2026lotgd}} & \rotatebox{90}{TravianZ~\cite{shadowss2026travianz}} & \rotatebox{90}{2Moons~\cite{kroepke20192moons}} & \rotatebox{90}{BrowserQuest~\cite{mozilla2012browserquest}} & \rotatebox{90}{Dragon Knight~\cite{seven2006dragonknight}} & \rotatebox{90}{ezRPG~\cite{ezrpg2016ezrpg}} \\
\midrule
Tile world map & $\bullet$ & $\bullet$ &  & $\bullet$ &  & $\bullet$ & $\bullet$ &  \\
Minimap around the player & $\bullet$ & $\bullet$ &  & $\bullet$ &  & $\circ$ &  &  \\
Map decoration from a coordinate hash & $\bullet$ &  &  &  &  &  &  &  \\
Fog of war & $\bullet$ &  &  &  &  &  &  &  \\
Enemy level grows with distance & $\bullet$ &  &  &  &  &  & $\bullet$ &  \\
Bank for items & $\bullet$ &  &  &  &  &  &  &  \\
Money transfer between players & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ &  &  &  \\
Item transfer between players & $\bullet$ &  &  & $\circ$ &  &  &  &  \\
Two-sided trade with confirmation & $\bullet$ &  &  & $\circ$ &  &  &  &  \\
Turn-based duel, both players online & $\bullet$ & $\bullet$ & $\circ$ &  &  &  &  &  \\
Item durability & $\bullet$ &  &  &  &  &  &  &  \\
Alchemy or crafting & $\bullet$ &  &  &  &  &  &  &  \\
Chat per map coordinate & $\bullet$ &  & $\circ$ &  &  & $\circ$ &  &  \\
Interface in more than one language & $\bullet$ &  & $\circ$ & $\bullet$ & $\bullet$ &  &  & $\bullet$ \\
Anti-forgery tokens on forms & $\bullet$ &  & $\bullet$ & $\bullet$ & $\circ$ &  &  &  \\
Layout for small screens & $\bullet$ & $\bullet$ & $\bullet$ &  & $\circ$ & $\bullet$ &  &  \\
Server push (WebSocket or SSE) &  &  & $\circ$ &  & $\circ$ & $\bullet$ &  &  \\
Clans, guilds or alliances & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ &  &  &  \\
\midrule
Features present, of 57 & 50 & 29 & 28 & 21 & 11 & 8 & 14 & 6 \\
\bottomrule
\end{tabular}
\begin{tablenotes}
\item $^{*}$ System presented in this work. $\bullet$ present, $\circ$ partial, blank absent. The last row counts the features marked present among the 57 features surveyed, of which the table shows a selection.
\end{tablenotes}
\end{table}


==> tables/systems.tex <==
\begin{table*}[t]
\centering
\caption{Open-source browser games in comparison and the size of their source code.}
\label{tab:systems}
\begin{tabular}{llrrrrrr}
\toprule
System & Genre & Files & Code & Comment & Blank & Declared & Bundled \\
\midrule
\textbf{Nigeru~RPG}$^{*}$ & RPG & 148 & 25,930 & 2,528 & 4,020 & 0 & 0 \\
Shinobi Chronicles~\cite{elementum2026shinobi} & RPG & 575 & 117,448 & 11,346 & 15,244 & 2 & 3 \\
Legend of the Green Dragon~\cite{nbcore2026lotgd} & RPG & 578 & 81,506 & 15,049 & 10,365 & 8 & 2,068 \\
TravianZ~\cite{shadowss2026travianz} & strategy & 1,164 & 167,548 & 17,343 & 23,533 & 0 & 1 \\
2Moons~\cite{kroepke20192moons} & strategy & 973 & 141,151 & 30,171 & 18,366 & 0 & 235 \\
ezRPG~\cite{ezrpg2016ezrpg} & RPG engine & 491 & 36,926 & 18,282 & 7,025 & 0 & 204 \\
Dragon Knight~\cite{seven2006dragonknight} & RPG & 35 & 4,771 & 79 & 708 & 0 & 0 \\
BrowserQuest~\cite{mozilla2012browserquest} & action RPG & 82 & 27,405 & 3,071 & 5,417 & 7 & 0 \\
\bottomrule
\end{tabular}
\begin{tablenotes}
\item $^{*}$ System presented in this work. Files are the source files with the extensions php, inc, js, css, html, htm, tpl, sql, py and sh, outside vendored libraries, tests and documentation. Code, Comment and Blank are the numbers of lines of each class. Declared is the number of third-party packages required by the package manifests of the repository, and Bundled the number of third-party library files kept in it.
\end{tablenotes}
\end{table*}


==> tables/u1.tex <==
\begin{table}[t]
\centering
\caption{Accessibility of the pages of each game after the login, in the desktop viewport.}
\label{tab:u1}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lrrrrrr}
\toprule
Game & Pages & Rules & Viol. & Severe & Elements & Small (\%) \\
\midrule
\textbf{Nigeru}$^{*}$ & 6 & 4 & 16 & 16 & 142 & 48.0 \\
Shinobi & 7 & 5 & 30 & 30 & 224 & 53.0 \\
LotGD & 2 & 0 & 0 & 0 & 0 & 16.7 \\
TravianZ & 5 & 6 & 17 & 17 & 97 & 64.6 \\
\bottomrule
\end{tabular}
\begin{tablenotes}
\item $^{*}$ System presented in this work. Rules is the number of distinct rules violated, Viol. the violations summed over the pages, Severe those classified as critical or serious, Elements the failing elements and Small the percentage of interactive elements below the minimum target size.
\end{tablenotes}
\end{table}


==> tables/u2.tex <==
\begin{table}[t]
\centering
\caption{Time predicted by the Keystroke-Level Model for each task, in seconds, with the number of page loads in parentheses.}
\label{tab:u2}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lrrrr}
\toprule
Task & \textbf{Nigeru}$^{*}$ & Shinobi & LotGD & TravianZ \\
\midrule
Log in & 9.6 (1) & \textbf{9.4 (1)} & 11.5 (1) & 10.0 (2) \\
Move one tile & \textbf{2.9 (1)} & 5.4 (3) &  &  \\
Attack once & \textbf{2.9 (1)} & 10.9 (5) & 13.5 (3) &  \\
Open character sheet & 2.7 (0) & \textbf{0.0 (0)} & \textbf{0.0 (0)} & 3.2 (2) \\
Buy an item & 8.6 (3) & \textbf{8.1 (3)} & 9.1 (2) &  \\
Deposit money & \textbf{8.7 (2)} &  & 16.4 (3) &  \\
Withdraw money & \textbf{9.0 (2)} &  & 16.1 (3) &  \\
Send money to a player & \textbf{14.6 (3)} & 17.7 (4) & 23.5 (4) &  \\
Read a private message & \textbf{2.9 (1)} & 5.5 (4) &  & 6.3 (4) \\
Send a private message & \textbf{15.6 (2)} & 18.0 (4) &  & 23.0 (6) \\
\bottomrule
\end{tabular}
\begin{tablenotes}
\item $^{*}$ System presented in this work. A blank cell is a task the game does not offer. Bold marks the shortest time among the games that offer the task. In Shinobi Chronicles and Legend of the Green Dragon the character sheet is already on the page reached after the login, so the task needs no action.
\end{tablenotes}
\end{table}

